A Quic(k) Security Overview: A Literature Research on Implemented Security Recommendations

Built on top of UDP, the relatively new QUIC protocol serves as the baseline for modern web protocol stacks. Equipped with a rich feature set, the protocol is defined by a 151 pages strong IETF standard complemented by several additional documents. Enabling fast updates and feature iteration, most QUIC implementations are implemented as user space libraries leading to a large and fragmented ecosystem. This work addresses the research question, "if a complex standard with a large number of different implementations leads to an insecure ecosystem?". The relevant RFC documents were studied and "Security Consideration" items describing conceptional problems were extracted. During the research, 13 popular production ready QUIC implementations were compared by evaluating 10 security considerations from RFC9000. While related studies mostly focused on the functional part of QUIC, this study confirms that available QUIC implementations are not yet mature enough from a security point of view.

==> acronyms.tex <==
\newacronym{tls}{TLS}{Transport Layer Security}
\newacronym{tcp}{TCP}{Transmission Control Protocol}
\newacronym{udp}{UDP}{User Datagram Protocol}
\newacronym{http}{HTTP}{Hypertext Transfer Protocol}
\newacronym{ietf}{IETF}{Internet Engineering Task Force}
\newacronym{ecn}{ECN}{Explicit Congestion Notification}
\newacronym{foss}{FOSS}{Free and open-source software}
\newacronym{dns}{DNS}{Domain Name System}
\newacronym{api}{API}{Application Programming Interface}

